Towards trustworthy agentic AI: a comprehensive survey of safety, robustness, privacy, and system security

Agentic AI systems -- Large Language Models (LLMs) augmented with planning, tool use, memory, and long-horizon interactions -- can execute complex tasks autonomously, but their multi-step trajectories introduce new failure modes that challenge trustworthiness. This survey provides a focused examination of trustworthy agentic AI through two core dimensions that are critical for high-risk deployments: Safety and Robustness, and Privacy and System Security. For each dimension, we clarify key concepts, identify where risks emerge along the agent workflow, and summarize stage-targeted mitigation strategies. Other trustworthiness aspects (value alignment, transparency, fairness, and accountability) are discussed as relevant context rather than parallel chapters. To support consistent comparison and deployment decisions, we consolidate evaluation into a unified metrics-and-benchmarks hub, emphasizing both outcome and process signals (e.g., constraint violations, trace completeness, and adversarial success rates) and offering scenario-to-metric guidance for release gating. We conclude by outlining open challenges such as self-evolving agents, runtime monitoring and verification, privacy-preserving personalization, and the trust-utility trade-off, and present a case study of real-world security failures in open-source agentic systems. Our goal is to serve as a practical reference for researchers and practitioners building trustworthy agentic systems in high-stakes environments.

==> Definitions/journalnames.tex <==
% Updated 14 November 2024
%\DeclareOption{}{\gdef\@journalweb{}\gdef\@journalfull{}\gdef\@journalshort{}\gdef\@doiabbr{}\gdef\@ISSN{}}
%% Website Name	%%	% Website Name	%% Full Name	%% Short Name	%% DOI abbr	%% ISSN

%1
\DeclareOption{Acad.Biol.}{\gdef\@journal{acadbiol}\gdef\@journalweb{academia-biology}\gdef\@journalfull{ACADEMIA BIOLOGY}\gdef\@journalfullname{Academia Biology}\gdef\@journalshort{Acad. Biol.}\gdef\@doiabbr{AcadBiol}\gdef\@ISSN{2837-4010}}
%2
\DeclareOption{Acad.Energy.}{\gdef\@journal{acadenergy}\gdef\@journalweb{academia-green-energy}\gdef\@journalfull{ACADEMIA GREEN ENERGY}\gdef\@journalfullname{Academia Green Energy}\gdef\@journalshort{Acad. Energy.}\gdef\@doiabbr{AcadEnergy}\gdef\@ISSN{2998-3665}}
%3
\DeclareOption{Acad.Eng.}{\gdef\@journal{acadeng}\gdef\@journalweb{academia-engineering}\gdef\@journalfull{ACADEMIA ENGINEERING}\gdef\@journalfullname{Academia Engineering}\gdef\@journalshort{Acad. Eng.}\gdef\@doiabbr{AcadEng}\gdef\@ISSN{2994-7065}}
%4
\DeclareOption{Acad.Env.Sci.Sust.}{\gdef\@journal{acadenvscisust}\gdef\@journalweb{academia-environmental-sciences-and-sustainability}\gdef\@journalfull{ACADEMIA ENVIRONMENTAL SCIENCES AND SUSTAINABILITY}\gdef\@journalfullname{Academia Environmental Sciences and Sustainability}\gdef\@journalshort{Acad. Env. Sci. Sust.}\gdef\@doiabbr{AcadEnvSciSust}\gdef\@ISSN{2997-6006}}
%5
\DeclareOption{Acad.Mat.Sci.}{\gdef\@journal{acadmatsci}\gdef\@journalweb{academia-materials-science}\gdef\@journalfull{ACADEMIA MATERIALS SCIENCE}\gdef\@journalfullname{Academia Materials Science}\gdef\@journalshort{Acad. Mat. Sci.}\gdef\@doiabbr{AcadMatSci}\gdef\@ISSN{2997-2027}}
%6
\DeclareOption{Acad.Med.}{\gdef\@journal{acadmedhealth}\gdef\@journalweb{academia-medicine-and-health}\gdef\@journalfull{ACADEMIA MEDICINE AND HEALTH}\gdef\@journalfullname{Academia Medicine and Health}\gdef\@journalshort{Acad. Med. Health.}\gdef\@doiabbr{AcadMedHealth}\gdef\@ISSN{3070-3530}}
%7
\DeclareOption{Acad.Ment.Health.WellB.}{\gdef\@journal{acadmenthealthwellb}\gdef\@journalweb{academia-mental-health-and-well-being}\gdef\@journalfull{ACADEMIA MENTAL HEALTH AND WELL-BEING}\gdef\@journalfullname{Academia Mental Health and Well-Being}\gdef\@journalshort{Acad. Ment. Health WellB.}\gdef\@doiabbr{AcadMentHealthWellB}\gdef\@ISSN{2997-9196}}
%8
\DeclareOption{Acad.Mol.Biol.Genom.}{\gdef\@journal{acadmolbiolgenom}\gdef\@journalweb{academia-molecular-biology-and-genomics}\gdef\@journalfull{ACADEMIA MOLECULAR BIOLOGY AND GENOMICS}\gdef\@journalfullname{Academia Molecular Biology and Genomics}\gdef\@journalshort{Acad. Mol. Biol. Genom.}\gdef\@doiabbr{AcadMolBiolGenom}\gdef\@ISSN{3064-9765}}
%9
\DeclareOption{Acad.NanoSci.Mat.Tech.}{\gdef\@journal{acadnanoscimattech}\gdef\@journalweb{academia-nano-science-materials-technology}\gdef\@journalfull{ACADEMIA NANO: SCIENCE, MATERIALS, TECHNOLOGY}\gdef\@journalfullname{Academia Nano: Science, Materials, Technology}\gdef\@journalshort{Acad. Nano: Sci. Mat. Tech.}\gdef\@doiabbr{AcadNanoSciMatTech}\gdef\@ISSN{3065-9736}}
%10
\DeclareOption{Acad.Nutri.}{\gdef\@journal{acadnutri}\gdef\@journalweb{academia-nutrition-and-dietetics}\gdef\@journalfull{ACADEMIA NUTRITION AND DIETETICS}\gdef\@journalfullname{Academia Nutrition and Dietetics}\gdef\@journalshort{Acad. Nutri.}\gdef\@doiabbr{AcadNutri}\gdef\@ISSN{3067-1345}}
%11
\DeclareOption{Acad.Oncol.}{\gdef\@journal{acadoncol}\gdef\@journalweb{academia-oncology}\gdef\@journalfull{ACADEMIA ONCOLOGY}\gdef\@journalfullname{Academia Oncology}\gdef\@journalshort{Acad. Oncol.}\gdef\@doiabbr{AcadOncol}\gdef\@ISSN{2998-7741}}
%12
\DeclareOption{Acad.Quant.}{\gdef\@journal{acadquant}\gdef\@journalweb{academia-quantum}\gdef\@journalfull{ACADEMIA QUANTUM}\gdef\@journalfullname{Academia Quantum}\gdef\@journalshort{Acad. Quant.}\gdef\@doiabbr{AcadQuant}\gdef\@ISSN{3064-979X}}

\DeclareOption{Acad.Dis.}{\gdef\@journal{acaddis}\gdef\@journalweb{academia-immunity-and- disease}\gdef\@journalfull{ACADEMIA IMMUNITY AND DISEASE}\gdef\@journalfullname{Academia Immunity and Disease}\gdef\@journalshort{Acad. Dis.}\gdef\@doiabbr{AcadDis}\gdef\@ISSN{pending}}

\DeclareOption{Acad.Drug.}{\gdef\@journal{acaddrug}\gdef\@journalweb{academia-drug-development-and-pharmacotherapy}\gdef\@journalfull{ACADEMIA DRUG DEVELOPMENT AND PHARMACOTHERAPY}\gdef\@journalfullname{Academia Drug Development and Pharmacotherapy}\gdef\@journalshort{Acad. Drug.}\gdef\@doiabbr{AcadDrug}\gdef\@ISSN{3071-2521}}


\DeclareOption{Acad.AI.}{\gdef\@journal{acadai}\gdef\@journalweb{academia-ai-and-applications}\gdef\@journalfull{ACADEMIA AI AND APPLICATIONS}\gdef\@journalfullname{Academia AI and Applications}\gdef\@journalshort{Acad. AI.}\gdef\@doiabbr{AcadAI}\gdef\@ISSN{3071-0286}}

\DeclareOption{Acad.Neurosci.BrainRes.}{\gdef\@journal{acadneuroscibrainres}\gdef\@journalweb{academia-neuroscience-and-brain-research}\gdef\@journalfull{ACADEMIA NEUROSCIENCE AND BRAIN RESEARCH}\gdef\@journalfullname{Academia Neuroscience and Brain Research}\gdef\@journalshort{Acad. Neurosci. Brain Res.}\gdef\@doiabbr{AcadNeurosciBrainRes}\gdef\@ISSN{pending}}

\DeclareOption{Acad.Catal.}{\gdef\@journal{acadcatal}\gdef\@journalweb{academia-catalysis}\gdef\@journalfull{ACADEMIA CATALYSIS}\gdef\@journalfullname{Academia Catalysis}\gdef\@journalshort{Acad. Catal.}\gdef\@doiabbr{AcadCatal}\gdef\@ISSN{pending}}

\DeclareOption{Acad.Glob.PublicHealth.}{\gdef\@journal{acadglobpublichealth}\gdef\@journalweb{academia-global-and-public-health}\gdef\@journalfull{ACADEMIA GLOBAL AND PUBLIC HEALTH}\gdef\@journalfullname{Academia Global and Public Health}\gdef\@journalshort{Acad. Glob. Public Health.}\gdef\@doiabbr{AcadGlobPublicHealth}\gdef\@ISSN{3071-0324}}


\DeclareOption{AcademiaEarthPlanet.Sci.}{\gdef\@journal{acadearthsci}\gdef\@journalweb{academia-earth-and-planetary-science}\gdef\@journalfull{ACADEMIA EARTH AND PLANETARY SCIENCE}\gdef\@journalfullname{Academia Earth and Planetary Science}\gdef\@journalshort{Academia Earth Planet. Sci.}\gdef\@doiabbr{AcademiaEarthPlanetSci}\gdef\@ISSN{pending}}

\DeclareOption{Acad.Med.ImagingRadiat.Ther.}{\gdef\@journal{acadmedimaging}\gdef\@journalweb{academia-medical-imaging-and-radiation-therapy}\gdef\@journalfull{ACADEMIA MEDICAL IMAGING AND RADIATION THERAPY}\gdef\@journalfullname{Academia Medical Imaging and Radiation Therapy}\gdef\@journalshort{Acad. Med. Imaging Radiat. Ther.}\gdef\@doiabbr{Acad.Med.ImagingRadiat.Ther.}\gdef\@ISSN{pending}}

\DeclareOption{nojournal}{\gdef\@journal{acadquant}\gdef\@journalweb{academia-journal}\gdef\@journalfull{Academia Journal}\gdef\@journalfullname{}\gdef\@journalshort{Acad. J.}\gdef\@doiabbr{AcadJ}\gdef\@ISSN{pending}}


==> Figures/agentic_system_architecture.tex <==
\begin{tikzpicture}[
    node distance=2.5cm,
    font=\small\sffamily,
    % Styles
    box/.style={
        draw=black!60, 
        thick,
        rounded corners=4pt, 
        align=center, 
        minimum width=2.4cm, 
        minimum height=1.1cm, 
        fill=white, 
        drop shadow={opacity=0.15}, 
        inner sep=4pt
    },
    container/.style={
        draw=gray!50, 
        dashed, 
        thick,
        rounded corners=12pt, 
        inner sep=20pt,
        fill=gray!5
    },
    labelnode/.style={
        font=\bfseries\large, 
        text=black!80, 
        anchor=center,          
        fill=white,
        inner sep=5pt,
        text depth=0pt
    },
    % Line Styles
    controlflow/.style={
        ->, 
        >=stealth, 
        very thick, 
        rounded corners=4pt, 
        draw=black!80
    },
    dataflow/.style={
        ->, 
        >=stealth, 
        thick, 
        dashed, 
        rounded corners=4pt, 
        draw=gray!70
    },
    % Crossing Halo
    halo/.style={
        preaction={draw=white, line width=4pt}
    },
    hooklabel/.style={
        font=\scriptsize\bfseries, 
        text=red!60!black, 
        align=center, 
        fill=white, 
        inner sep=2pt,
        draw=red!20,
        rounded corners=2pt,
        thin,
        drop shadow={opacity=0.05}
    },
    % Edge label style
    edgelabel/.style={
        font=\scriptsize,
        fill=white,
        inner sep=1.5pt
    }
]
    % --- Components within the Agent ---
    % Memory (0, 3.5), World Model (5, 3.5)
    \node[box, fill=harvestgold!15] (memory) at (0, 3.5) {\textbf{Memory}\\\scriptsize(Episodic, Semantic)};
    \node[box, fill=capri!15] (worldmodel) at (5, 3.5) {\textbf{World Model}\\\scriptsize(Simulator, Predictor)};

    % Perceive (0, 0), Plan (5, 0), Act (10, 0)
    \node[box, fill=brightlavender!15] (perceive) at (0, 0) {\textbf{Perceive}\\\scriptsize($s_t \leftarrow o_t$)};
    \node[box, fill=lightgreen!15] (plan) at (5, 0) {\textbf{Plan}\\\scriptsize(Decompose, Reason)};
    \node[box, fill=lightcoral!15] (act) at (10, 0) {\textbf{Act}\\\scriptsize(Tools, API)};
    
    % Reflect (5, -3.5)
    \node[box, fill=plum!15] (reflect) at (5, -3.5) {\textbf{Reflect} \& \textbf{Learn}\\\scriptsize(Eval, Update)};


    % --- Container & Title ---
    \begin{scope}[on background layer]
        \node[container, fit=(memory) (worldmodel) (perceive) (act) (reflect) (plan), minimum height=9.5cm, minimum width=13.5cm] (agentbox) {};
    \end{scope}
    
    % Title on the border - CENTERED
    \node[labelnode] at (agentbox.north) {Agent System};


    % --- External Entities ---
    % Human (x=-5, y=3.5)
    \node[draw=black!60, thick, circle, fill=white, minimum size=1.6cm, align=center, drop shadow={opacity=0.15}] (human) at (-5.0, 3.5) {Human\\Admin};
    
    % Environment (x=14, y=0)
    \node[draw=black!60, thick, rounded corners=6pt, fill=blue!5, minimum width=2.4cm, minimum height=5cm, align=center, drop shadow={opacity=0.15}] (env) at (15, 0) {\textbf{Environment}\\\scriptsize(External Systems)};


    % --- Connections ---

    % 1. Human Inputs to Memory (Goals, Constraints, and Budget)
    \draw[controlflow] (human) -- node[midway, above, align=center, font=\scriptsize] {Goals ($G$),\\Constraints ($K$),\\Budget ($B$)} (memory.west);
    
    % Human Oversight to Perceive
    \draw[controlflow, gray] (human.south) |- node[pos=0.7, above, font=\scriptsize] {Oversight} (perceive.west);


    % 2. Internal Data Flow (Dashed) -- with labels
    % Memory -> Perceive: Recall
    \draw[dataflow] (memory.south) -- node[right, edgelabel, pos=0.5] {Recall} (perceive.north);
    % Perceive -> Memory: Store
    \draw[dataflow] ([xshift=-1cm]perceive.north) -- node[left, edgelabel, pos=0.5] {Store} ([xshift=-1cm]memory.south);

    % Memory -> Plan: Context
    \draw[dataflow] (memory.south east) -- node[left, edgelabel, pos=0.3] {Context} (plan.north west);
    
    % World Model -> Plan: Predicted outcomes (key reviewer request)
    \draw[dataflow] ([xshift=-5pt]worldmodel.south) -- node[left, edgelabel, pos=0.5] {\shortstack{Predicted\\outcomes}} ([xshift=3pt]plan.north);
    % Plan -> World Model: Candidate plans for simulation
    \draw[dataflow] ([xshift=10pt]plan.north east) -- node[right, edgelabel, pos=0.4] {\shortstack{Candidate\\plans}} (worldmodel.south east);


    % 3. Main Execution Loop -- with labels
    % Perceive -> Plan: observation o_t (reviewer: observation should be Perceive->Plan)
    \draw[controlflow] (perceive) -- node[above, edgelabel] {Observation ($o_t$)} (plan);
    
    % Plan -> Act: action a_t
    \draw[controlflow] (plan) -- node[above, edgelabel] {Action ($a_t$)} (act);
    \node[hooklabel, below=3pt] at (7.5, 0) {Safeguards};
    
    % Act -> Environment: tool calls / API invocations
    \draw[controlflow] (act) -- node[above, edgelabel, pos=0.5] {Tool calls} (env);

    % Environment -> Perceive: state s_t (reviewer: this should be state, not observation)
    \draw[controlflow] (env.south) -- ++(0, -4.2) -| node[near start, below, font=\scriptsize] {State ($s_t$)} (perceive.south);


    % 4. Reflection Loop & High Road Routing -- with labels
    % Act -> Reflect: outcome/result (reviewer: arrow direction was missing)
    \draw[controlflow] (act.south) |- node[pos=0.25, right, edgelabel] {Outcome} ([yshift=4pt]reflect.east);
    % Environment -> Reflect: reward signal
    \draw[controlflow] (env.south) |- node[pos=0.1, below, edgelabel] {Reward ($r_t$)} (9, -3.8) -- ([yshift=-4pt]reflect.east);
    % Reflect -> Plan: revised plan / feedback
    \draw[controlflow] (reflect.north) -- node[left, edgelabel] {Feedback} (plan.south);
    
    % Reflect -> Memory (Update)
    % "The High Road" - Reflect -> right -> up -> left -> Memory
    \draw[controlflow, halo] (reflect.east) -- (13.0, -3.5) -- (13.0, 5.8) -- node[above, edgelabel] {Update} (0, 5.8) -- (memory.north);

    
    % 5. Assurance Labels
    \node[hooklabel] at (1.8, 2.2) {Validation};
    \node[hooklabel] at (9.0, 0.8) {Verification};
    \node[hooklabel] at (4.0, -1.75) {Diagnostics};
    \node[hooklabel, anchor=south west] at (reflect.south east) {Logging};

\end{tikzpicture}


==> Figures/cross_domain_lifecycle.tex <==

\begin{table*}[htbp]
\centering
\caption{Cross-domain mapping of core trustworthiness dimensions. Each cell summarizes the domain-specific challenges and mitigation methods with supporting references. This table focuses on the two core dimensions critical for high-risk deployments: Safety \& Robustness and Privacy \& System Security.}
\label{fig:comparison_framework}
\renewcommand{\arraystretch}{1.5}
\setlength{\tabcolsep}{4pt}
\scriptsize
\begin{tabularx}{\linewidth}{@{} >{\raggedright\arraybackslash\bfseries}p{2.1cm} >{\raggedright\arraybackslash}X >{\raggedright\arraybackslash}X >{\raggedright\arraybackslash}X @{}}
\toprule
\textbf{Dimension} & \textbf{Autonomous Driving (AD)} & \textbf{Healthcare (HC)} & \textbf{Intelligent Assistants (IA)} \\
\midrule

\rowcolor{brightlavender!15}
Safety \& Robustness 
& \textit{Challenge:} Perception failures in adverse weather, occlusion, long-tail scenarios; collision prevention.

\textit{Methods:} V2X collaborative sensing, simulation-based validation, Safe RL, runtime shielding~\citep{a17030103,ZHAO2024122836,yao2025agentsllmaugmentativegenerationchallenging}.
& \textit{Challenge:} Diagnostic errors, clinical decision failures, hazardous hallucinations.

\textit{Methods:} Multi-center validation, clinician-in-the-loop architecture, uncertainty quantification~\citep{diagnostics14141472,udegbe2024role,healthcare12020125}.
& \textit{Challenge:} Tool execution failures, indirect prompt injection, memory poisoning.

\textit{Methods:} Sandboxed execution, LM-emulated testing, input sanitization~\citep{ruan2024identifyingriskslmagents,NEURIPS2024_97091a51,yu2025survey}. \\

\rowcolor{carminepink!15}
Privacy \& System Security
& \textit{Challenge:} V2X data exposure, location tracking, cybersecurity threats (spoofing, jamming).

\textit{Methods:} Secure V2X protocols, ISO/SAE 21434 compliance, data anonymization~\citep{ZHAO2024122836,J3016_202104}.
& \textit{Challenge:} Patient data breaches, re-identification risks, EHR security.

\textit{Methods:} HIPAA/GDPR compliance, federated learning, end-to-end encryption~\citep{bioengineering11040337,life14050557}.
& \textit{Challenge:} Credential theft, unauthorized tool access, data exfiltration.

\textit{Methods:} Least-privilege access, ephemeral credentials, policy enforcement, audit logging~\citep{yu2025survey,limind,NEURIPS2024_97091a51}. \\

\bottomrule
\end{tabularx}
\end{table*}


==> Figures/paper_structure.tex <==
\begin{figure*}[t]
  \centering
  \begin{tikzpicture}[
    node distance=0.6cm and 0.3cm,
    section/.style={draw, rounded corners=4pt, minimum height=0.7cm, font=\small\bfseries, align=center},
    subsec/.style={draw, rounded corners=3pt, minimum height=0.7cm, font=\tiny, align=center},
    arrow/.style={->, >=stealth, thick, gray},
    label/.style={font=\tiny\itshape, text=gray}
  ]
    
    % Constants for layout
    \def\totalwidth{13.5cm}
    \def\rowgap{0.6cm}
    
    %% Section 1: Introduction (Anchor for width)
    \node[section, fill=gray!20, minimum width=\totalwidth] (intro) {\hyperref[section:introduction]{Section~1 Introduction}};
    % Label moved to end to avoid being covered by arrow
    
    %% Section 2: Preliminaries
    \node[section, fill=brightlavender!25, below=\rowgap of intro, minimum width=\totalwidth] (prelim) {\hyperref[section:preliminaries]{Section~2 Preliminaries: Agentic AI \& Workflow}};
    
    % Sub-sections of S2 (3 boxes)
    \def\s2width{4.3cm}
    \node[subsec, fill=brightlavender!15, below=0.4cm of prelim.south, minimum width=\s2width] (s22) {\hyperref[sec:rl-coupling]{Section~2.2 RL \& Preference}\\Optimization Foundations};
    \node[subsec, fill=brightlavender!15, left=0.3cm of s22, minimum width=\s2width] (s21) {\hyperref[sec:preliminaries-agentic]{Section~2.1 Definition \& Components}\\Perceive$\to$Plan$\to$Act$\to$Reflect$\to$Learn};
    \node[subsec, fill=brightlavender!15, right=0.3cm of s22, minimum width=\s2width] (s23) {\hyperref[sec:risk-assurance]{Section~2.3 Risk Surface \&}\\Assurance Stack};
    
    %% Section 3: Core Dimensions (Updated for 2 dimensions)
    \node[section, fill=lightgreen!25, below=0.8cm of s22, minimum width=\totalwidth] (coredim) {\hyperref[section:core_dimensions]{Section~3 Core Dimensions of Trustworthiness}};
    
    % 2 dimensions (instead of 6)
    \def\dgap{0.5cm}
    \def\dwidth{5.5cm}
    
    % Positioning relative to center - two boxes side by side
    \node[subsec, fill=brightlavender!20, below=0.4cm of coredim.south, xshift=-3cm, minimum width=\dwidth, text width=5.3cm] (d1) {\hyperref[subsection:safety]{Safety \& Robustness}\\Perceive$\to$Plan$\to$Act$\to$Reflect$\to$Learn};
    \node[subsec, fill=carminepink!20, below=0.4cm of coredim.south, xshift=3cm, minimum width=\dwidth, text width=5.3cm] (d2) {\hyperref[subsection:privacy]{Privacy \& System Security}\\Perceive$\to$Plan$\to$Act$\to$Reflect$\to$Learn};
    
    %% Section 4
    \def\row5gap{0.5cm}
    \def\row5width{\totalwidth}
    
    % ABSOLUTE POSITIONING relative to intro center for perfect symmetry
    \path (d1.south) ++(0, -1.0cm) coordinate (row5_y);
    
    % Section 4 centered with full width
    \node[section, fill=lightyellow!40, minimum width=\row5width, anchor=north] (eval) at (intro.center |- row5_y) {\hyperref[section:eval]{Section~4 Metrics \& Benchmarks}};
    
    % Content box
    \node[subsec, fill=lightyellow!25, below=0.15cm of eval, minimum width=\row5width, text width=13cm] (eval_sub) {Metric Dictionary, Scenario-to-Metric Mapping, Evaluation Pipeline, Reporting Standards};
    
    %% Section 5: Challenges (renumbered from 6)
    % Single definition strictly centered
    \node[section, fill=gray!25, minimum width=\totalwidth, anchor=north] (challenges) at (intro.center |- eval_sub.south) [yshift=-0.6cm] {\hyperref[subsection:challenges]{Section~5 Challenges and Solutions}};
    
    %% Arrows
    \draw[arrow] (intro.south) -- (prelim.north);
    \draw[arrow] (prelim.south) -- (s22.north);
    \draw[arrow] (prelim.south) -- ++(0,-0.2) -| (s21.north);
    \draw[arrow] (prelim.south) -- ++(0,-0.2) -| (s23.north);
    
    \draw[arrow] (s22.south) -- (coredim.north);
    
    \draw[arrow] (coredim.south) -- ++(0,-0.4); % Short arrow down
    
    % Dimension arrows (2 dimensions)
    \draw[arrow] (coredim.south) -- ++(0,-0.15) -| (d1.north);
    \draw[arrow] (coredim.south) -- ++(0,-0.15) -| (d2.north);
    
    % Dashed dependency arrow from dimensions to eval
    \draw[arrow, dashed] (d1.south) -- ++(0,-0.4) -| ([xshift=-3cm]eval.north);
    \draw[arrow, dashed] (d2.south) -- ++(0,-0.4) -| ([xshift=3cm]eval.north);
    
    \draw[arrow] (eval_sub.south) -- (challenges.north);
    
    %% LABELS drawn last to be on top
    % 1. Introduction label
    \node[label, fill=white, inner sep=2pt, anchor=center] at (intro.center |- intro.south) [yshift=-0.3cm] {Motivation, Scope, Contributions};
    
    % 2. Dimensions note
    \node[label, fill=white, inner sep=2pt, anchor=center] (struct_note) at (intro.center |- d1.south) [yshift=-0.4cm] {Each: Definition $\to$ Risks $\to$ Methods (stage-aligned)};
    \draw[arrow] (coredim.south) -- (struct_note.north);

  \end{tikzpicture}
  \caption{Paper structure and reading guide. The survey begins with motivation and agentic AI preliminaries (Section~\ref{section:introduction}~--~\ref{section:preliminaries}~), then presents two core trustworthiness dimensions---Safety \& Robustness and Privacy \& System Security---with consistent Definition$\to$Risks$\to$Methods structure (Section~\ref{section:core_dimensions}~). Evaluation metrics consolidate process- and outcome-level assessments (Section~\ref{section:eval}~). Challenges and solutions conclude the survey (Section~\ref{subsection:challenges}~).}
  \label{fig:paper-structure}
\end{figure*}


==> Figures/taxonomy.tex <==

\FloatBarrier
\begin{figure*}[!htbp]
  \centering
  \resizebox{\linewidth}{!}{%
  \tikzset{
          my node/.style={
              draw,
              align=center,
              thin,
              text width=1.0cm, 
              rounded corners=2,
          },
          my leaf/.style={
              draw,
              align=left,
              thin,
              text width=5.5cm, 
              rounded corners=2,
          }
  }
  \forestset{
    every leaf node/.style={
      if n children=0{#1}{}
    },
    every tree node/.style={
      if n children=0{minimum width=1em}{#1}
    },
  }
  \begin{forest}
      nonleaf/.style={font=\bfseries\tiny},
       for tree={%
          every leaf node={my leaf, font=\tiny},
          every tree node={my node, font=\tiny, l sep-=5pt, l-=1.5pt},
          anchor=west,
          inner sep=2pt,
          l sep=8pt,
          s sep=1pt,
          fit=tight,
          grow'=east,
          edge={ultra thin},
          parent anchor=east,
          child anchor=west,
          if n children=0{}{nonleaf}, 
          edge path={
              \noexpand\path [draw, \forestoption{edge}] (!u.parent anchor) -- +(5pt,0) |- (.child anchor)\forestoption{edge label};
          },
          if={isodd(n_children())}{
              for children={
                  if={equal(n,(n_children("!u")+1)/2)}{calign with current}{}
              }
          }{}
      }
      [Trustworthy\\Agentic\\AI, draw=gray, fill=gray!15, text width=1.5cm, text=black
      %% ===== Safety & Robustness =====
      %% ORDER: matches Section 3.1.3 text order exactly
      [Safety \&\\Robustness\\({\cref{subsection:safety}}), color=brightlavender, fill=brightlavender!15, text width=1.9cm, text=black
            [Perceive, color=brightlavender, fill=brightlavender!15, text width=1.0cm, text=black
            [{Data augmentation, adversarial training, OOD detection, input provenance/sanitization, DRO objectives~\citep{yadgaroff2024improvinggeneralizationgameagents,HarmBench,10.5555/3545946.3598721,Sagawa2020GroupDRO}
                }, color=brightlavender, fill=brightlavender!15, text=black]
            ]
            [Plan, color=brightlavender, fill=brightlavender!15, text width=1.0cm, text=black
            [{Safe RL (CMDPs/CPO), CVaR objectives, constitutional constraints, conservative/specification-aware planning~\citep{Altman1999,Achiam2017CPO,bai2022constitutional,kushwaha2025surveysafereinforcementlearning}
                }, color=brightlavender, fill=brightlavender!15, text=black]
            ]
            [Act, color=brightlavender, fill=brightlavender!15, text width=1.0cm, text=black
            [{Guardrails, runtime shielding, least-privilege tools, sandboxing, transactional execution, HITL approval~\citep{10.5555/3504035.3504361,zheng2025webguardbuildinggeneralizableguardrail,NIST2023RMF}
                }, color=brightlavender, fill=brightlavender!15, text=black]
            ]
            [Reflect, color=brightlavender, fill=brightlavender!15, text width=1.0cm, text=black
            [{Simulation-based testing, red teaming, trace auditing, formal verification of components~\citep{10.1109/ICSE55347.2025.00223,HarmBench,4567924}
                }, color=brightlavender, fill=brightlavender!15, text=black]
            ]
            [Learn, color=brightlavender, fill=brightlavender!15, text width=1.0cm, text=black
            [{Regression gating, canary rollouts, conservative safe policy improvement, incident-driven datasets~\citep{Sculley2015HiddenDebt,Breck2017MLTestScore,Burns2018SpinnakerCD,Laroche2019SPIBB}
                }, color=brightlavender, fill=brightlavender!15, text=black]
            ]
            [Multi-\\agent, color=brightlavender, fill=brightlavender!15, text width=1.0cm, text=black
            [{Protocol-level constraints, agent authentication, centralized oversight/governors, global budget enforcement~\citep{Dafoe2020Cooperative}
                }, color=brightlavender, fill=brightlavender!15, text=black]
            ]
            [Long-\\horizon, color=brightlavender, fill=brightlavender!15, text width=1.0cm, text=black
            [{Hierarchical decomposition, checkpointing, risk budgets, receding-horizon replanning, interruptibility~\citep{Amodei2016Concrete}
                }, color=brightlavender, fill=brightlavender!15, text=black]
            ]
          ]
        %% ===== Privacy & System Security =====
        [Privacy \&\\System Security\\({\cref{subsection:privacy}}), color=carminepink, fill=carminepink!15, text width=1.9cm, text=black
              [Perceive, color=carminepink, fill=carminepink!15, text width=1.0cm, text=black
                [{Input sanitization, zero-trust intake, prompt injection detection~\citep{zhang2025searching,du2025beyond,nist2020zerotrust}
                    }, color=carminepink, fill=carminepink!15, text=black]
                ]
                [Plan, color=carminepink, fill=carminepink!15, text width=1.0cm, text=black
                [{Memory governance, contextual integrity, differential privacy, minimization~\citep{mireshghallah2025position,nissenbaum2004contextualintegrity,du2025beyond}
                    }, color=carminepink, fill=carminepink!15, text=black]
                ]
                [Act, color=carminepink, fill=carminepink!15, text width=1.0cm, text=black
                [{Sandboxing, credential vaulting, DLP filtering, runtime policy enforcement~\citep{zhang2025privweb,du2025beyond,zheng2025webguardbuildinggeneralizableguardrail}
                    }, color=carminepink, fill=carminepink!15, text=black]
                ]
                [Reflect, color=carminepink, fill=carminepink!15, text width=1.0cm, text=black
                [{Encrypted channels, authenticated provenance, tamper-evident logging~\citep{yang2025mla,mireshghallah2025position}
                    }, color=carminepink, fill=carminepink!15, text=black]
                ]
                [Learn, color=carminepink, fill=carminepink!15, text width=1.0cm, text=black
                [{Retention limits, supply chain controls (SBOMs), security regression gating~\citep{du2025beyond,spdx2021sbom,sigstore2022}
                    }, color=carminepink, fill=carminepink!15, text=black]
                ]
        ]
      ]
      \end{forest}
  }% end resizebox
  \caption{A hierarchical taxonomy of Trustworthy Agentic AI organized along two core trustworthiness dimensions: Safety \& Robustness and Privacy \& System Security. Each dimension is decomposed according to the five-stage agent lifecycle (Perceive$\to$Plan$\to$Act$\to$Reflect$\to$Learn). The Safety \& Robustness dimension additionally includes \textbf{Multi-agent} and \textbf{Long-horizon} branches, which address emergent coordination risks and compounding error beyond the single-agent, single-episode setting (see Sections~3.1.2--3.1.3). Leaf nodes list representative mitigation methods and key references, ordered consistently with the text in Section~3.}
  \label{fig: Taxonomy}
  \end{figure*}
\FloatBarrier
